Point-to-Point: Sparse Motion Guidance for Controllable Video Editing

Accurately preserving motion while editing a subject remains a core challenge in video editing tasks. Existing methods often face a trade-off between edit and motion fidelity, as they rely on motion representations that are either overfitted to the layout or only implicitly defined. To overcome this limitation, we revisit point-based motion representation. However, identifying meaningful points remains challenging without human input, especially across diverse video scenarios. To address this, we propose a novel motion representation, anchor tokens, that capture the most essential motion patterns by leveraging the rich prior of a video diffusion model. Anchor tokens encode video dynamics compactly through a small number of informative point trajectories and can be flexibly relocated to align with new subjects. This allows our method, Point-to-Point, to generalize across diverse scenarios. Extensive experiments demonstrate that anchor tokens lead to more controllable and semantically aligned video edits, achieving superior performance in terms of edit and motion fidelity.

==> tables/supp_trajectory.tex <==
\begin{table}[!h]
\footnotesize
\setlength{\tabcolsep}{0.1em}
\definecolor{Gray}{gray}{0.9}
\renewcommand{\arraystretch}{1.0}
\begin{tabularx}{\linewidth}{m{3cm} | Y Y Y}
    \toprule
    & ViCLIP $\uparrow$ & Flow Sim. $\uparrow$ & Warp Err. $\downarrow$ \\
    \midrule\midrule
    \(\kappa=1\) & & & \\ %0.243 & 0.719 & 0.317 \\
    \(\kappa=\lfloor \frac{N}{2} \rfloor\) & & & \\ %0.248 & 0.733 & 0.316 \\
    \(\kappa=N\) & & & \\ %0.249 & 0.700 & 0.309 \\
    Ours & \textbf{0.257} & 0.711 & 0.336  \\
    \bottomrule
\end{tabularx}
\caption{Ablation study on anchor token alignment.}
\vspace{-0.5\baselineskip}
\label{tbl:supp_trajectory}
\end{table}
---------------------------------------- %

